Less Is More: Tuning Configurable Systems with Imperfect Fidelity

Configuration tuning is essential for optimizing the performance of highly configurable systems, e.g., throughput or runtime, under a given environment. Yet, this is a challenging process as there can be many options to tune, and configuration measurement is often highly expensive. In this paper, we demonstrate the phenomenon of ``less can be more'': system configuration tuning can be greatly improved with much superior budget utilization by partially tuning under the imperfect-fidelity---an environment that is similar, but cheaper to measure, compared with the concerned perfect-fidelity of environment under which the system should be tuned. We codify a conceptual framework of fidelity for configurable systems, drawing on which allows us to propose MFTune, a tuner that proactively explores in the space of $>10^4$ possible imperfect-fidelity settings to approximate a useful one, which strikes for the wideness of tuning. This creates high-quality seeds for the perfect-fidelity, which in turn ensures the tuning depth. Experiment results against $10$ state-of-the-art tuners, obtained from running diverse real-world systems for $19$ months $24 \times 7$, show that MFTune performs considerably better on $83.33$\% cases with up to $19.34\%$ improvement while achieving hours of budget saving in general.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.16   Emergency release: fixes a typo in the code.

Version 2.15   Bug fixes.  Documentation updates
	       New journals: AILET, TAIS, TAISAP, ACMJDS

Version 2.14   Bib style update.  Documentation update.  DLT is now using
	       acmlarge format.
	       Generate error if a user tries to redefine sectioning commands

Version 2.13   Documentation update
	       Added mathcal in unicode mode
	       Bug fixes

Version 2.12   Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> paper_sections/method-bk.tex <==
\section{The \approach~Framework}
\label{section:methodology}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{figures/MFTune.pdf}
    \caption{Workflow overview of \approach.\tao{we might simplify this to contain only the main flow, leave details to more specific illustration.}}
    \label{fig:MFTune}
\end{figure}


\begin{table*}
	\centering
	\small
	%\tabcolsep=0.33 cm
	\caption{Key notations and their descriptions used in this work.}
        \label{tb:notation}
    \begin{adjustbox}{width=\linewidth,center}
	\begin{threeparttable}
		\input{tables/notation}
	\end{threeparttable}
     \end{adjustbox}
     \vspace{-5pt}
\end{table*}


Figure~\ref{fig:MFTune} and Algorithm~\ref{alg:mftune} illustrate the workflow of \approach. The key idea is to first explore the fidelity space to identify an ``ideal'' imperfect-fidelity setting---one that offers good fidelity perfection while incurring a much lower cost. Specifically designed diversity-preserving tuning would be conducted under the selected imperfect-fidelity setting for ``wide'' tuning, the process of which is also interleaved with the tuning under the perfect-fidelity setting for ``deep'' tuning. \approach~comprises the following key components:





%Figure 3 illustrates the workflow of MFTune, which builds on the characteristics identified in Section~\ref{subsection:motivation_challenges} and treats fidelity discovery and configuration tuning as two coupled problems. The key idea is to first explore the fidelity space to identify a cost-effective low-fidelity setting, one that offers high correlation with full-fidelity while incurring a much lower evaluation cost. As such, the fidelity setting can be used to guide tuning more efficiently. While theoretically applicable to different optimizers, we embed it into an evolutionary search framework, which naturally fits the staged multi-fidelity setting by supporting iterative population updates under varying fidelity levels. 

% that first accelerates exploration through low-fidelity evaluations and then refines promising regions under full-fidelity.

% While theoretically applicable to different optimizers, we embed it into an evolutionary search framework, enabling a staged process that combines rapid, low-cost exploration with precise refinement at full-fidelity. In this way, \approach~exploits low-fidelity to accelerate exploration and then concentrate the search on promising regions guided by full-fidelity evaluation.
%while strategically employing high-fidelity evaluations to keep the search aligned with the true objective. 


\begin{itemize}
    \item \textbf{Imperfect-Fidelity Discovering (line 3)} formulates an active, multi-objective fidelity discovery problem (maximize level of perfection while minimize cost) and applies NSGA-II~\cite{deb2002fast}---a common population-based multi-objective genetic algorithm---to evolve an ``ideal'' imperfect-fidelity setting (\textit{\textbf{Challenges 1}}).

    \item \textbf{Imperfect-Fidelity Seeding (line 4)} embeds the discovered imperfect-fidelity setting into the tuning, interleaving with the perfect-fidelity setting to verify the diversity-enforced configurations found, which covers a wide area of the space and generates high quality seeds for tuning under the pure perfect-fidelity setting. (\textit{\textbf{Challenge 2 and 3}}).

    \item \textbf{Perfect-Fidelity Assuring (line 5)} initializes the tuning from the seeded configurations obtained under imperfect-fidelity setting, hence fully exploiting the benefits from the tuning thereof for deeply exploring along the tuning directions implied (\textit{\textbf{Challenge 3}}).

    %This stage serves as the final safeguard, correcting potential biases introduced by low-fidelity proxy. By enforcing full-fidelity validation and evolution on promising candidates, it guarantees that the delivered configurations achieve deployment-grade reliability and practical usability 
\end{itemize}

Through proactively exploiting the benefits from the imperfect-fidelity settings, \approach~seeks to greatly improve the resource utilization when tuning configurable systems, leading to better efficiency and emergently promising results.
\tao{place marker; I fix till here.}
%\tao{If I am someone who does not know this approach before, I would be a bit struggle to understand how the low fidelity and high fidelity configs interacts; we might need to stress that point.}By integrating these components, \approach~decouples fidelity discovery from configuration tuning while tightly coupling them through staged evolutionary transitions. This design enables the framework to capitalize on low-fidelity evaluations for cost-effective exploration, progressively refine configurations under targeted full-fidelity setting, and ultimately deliver validated configurations. The overall procedures are summarized in \textbf{Algorithm~\ref{alg:mftune}}, with detailed designs of each component provided in Sections~\ref{subsection:EvoFD}-\ref{subsection:HiFEA}. Table~\ref{tb:notation} summarizes the key notations used throughout this work.

\input{paper_sections/pseudo_mftune}

\subsection{Discovering Ideal Imperfect-Fidelity}
\label{subsection:EvoFD}



EvoFD seeks to identify a low-fidelity setting $\boldsymbol{z}$ that can reflect configuration quality, to some extent, at a lower evaluation cost. As discussed in Section~\ref{subsection:motivation_challenges}, cost alone does not reliably indicate the fidelity level of a fidelity setting. We therefore quantify fidelity level based on the ranking consistency between low- and full-fidelity evaluations, using Spearman correlation ($\rho$)~\cite{wattanakriengkrai2022giving} as the metric. Spearman is chosen because it (i) evaluates ordering consistency, which is what drives selection in optimizers; (ii) is scale-free and less sensitive to outliers. To that end, EvoFD formulates fidelity discovery as a multi-objective optimization problem (i.e., maximize the fidelity level $\rho_{\boldsymbol{z}}$ while minimizing evaluation cost $\tau_{\boldsymbol{z}}$) and solves it with NSGA-II~\cite{deb2002fast} to expose Pareto-optimal trade-offs. As shown in Figure~\ref{fig:MFTune} and \textbf{Algorithm~\ref{alg:EvoFD}}, we perform the following:

\begin{itemize}
    \item[(1)] Generate a set $\boldsymbol{\mathcal{S}}$ = $\{\boldsymbol{x}_1, \dots, \boldsymbol{x}_l\}$ with $l$ diverse configurations via Latin Hypercube Sampling (LHS)~\cite{mckay1992latin} to provide a representative basis for fidelity quantification (line 2). 
    
    \item[(2)] Initialize a fidelity population $\boldsymbol{\mathbfcal{Q}}$ = \{$\boldsymbol{z}_1, \dots, \boldsymbol{z}_n$\} by randomly sampling $n$ candidate fidelity settings (line 3).
    
    \item [(3)] Measure fidelity population $\boldsymbol{\mathbfcal{Q}}$. For each candidate fidelity setting $\boldsymbol{z}$ $\in$ $\boldsymbol{\mathbfcal{Q}}$ , we can quantify its fidelity level \textcolor{red}{we can ref Eq 3} $\rho_{\boldsymbol{z}}$ and evaluation cost $\tau_{\boldsymbol{z}}$ by:
    \begin{equation}
    \label{eq:measure_fidelity}
    \begin{aligned}
    & \rho_{\boldsymbol{z}}=\operatorname{corr}(\mathbfcal{R}(\mathbfcal{F}_{\boldsymbol{z}}), \mathbfcal{R}(\mathbfcal{F}_{\boldsymbol{z}^*})), \\
    & \tau_{\boldsymbol{z}}=\frac{1}{l} \sum_{j=1}^l \tau_{\boldsymbol{z}}(\boldsymbol{x}_j), 
    \end{aligned}
    \end{equation}
    where $\mathbfcal{F}_{\boldsymbol{z}}$ = [$f_{\boldsymbol{z}}(\boldsymbol{x}_1)$, ..., $f_{\boldsymbol{z}}(\boldsymbol{x}_l)$] and $\mathbfcal{F}_{\boldsymbol{z}^*}$ = [$f_{\boldsymbol{z}^*}(\boldsymbol{x}_1)$, ..., $f_{\boldsymbol{z}^*}(\boldsymbol{x}_l)$] are the performance of all configurations $\boldsymbol{x}$ $\in$ $\boldsymbol{\mathcal{S}}$ under low-fidelity $\boldsymbol{z}$ and full-fidelity $\boldsymbol{z}^*$, respectively. $\mathbfcal{R}(\cdot)$ returns performance ranks, and $\tau_{\boldsymbol{z}}(\boldsymbol{x}_j)$ is the evaluation cost of $\boldsymbol{x}_j$ at fidelity setting $\boldsymbol{z}$ (line 4). 

    \item [(4)] Evolve the fidelity population using NSGA-II. In each generation, apply selection, crossover, and mutation operators to generate offspring $\boldsymbol{\mathbfcal{W}}$. Then, we can evaluate their fidelity levels and evaluation costs using Equation~(\ref{eq:measure_fidelity}), and update the population via non-dominated sorting~\cite{deb2002fast}. The process continues until the budget for fidelity discovery $\mathcal{B}_1$ is exhausted (lines 5-15). 

    \item [(5)] Select the most cost-effective non-dominated\footnote{A solution $\boldsymbol{z}_i$ (i.e., a fidelity setting) is dominated by $\boldsymbol{z}_j$ if all objectives of $\boldsymbol{z}_j$ are better or equivalent to those of $\boldsymbol{z}_i$ while there is at least one objective of $\boldsymbol{z}_j$ performs better than that of $\boldsymbol{z}_i$. A solution is said non-dominated if it cannot be dominated by any other solutions in this set.} fidelity setting from the final population as $\boldsymbol{z}_{ideal}$, defined by maximizing $\rho_{\boldsymbol{z}}$/$\tau_{\boldsymbol{z}}$ among the Pareto-optimal candidates (line 16). 
    
    %we measure all configurations \textbf{x} $\in$ $\boldsymbol{\mathcal{S}}$ under both \textbf{z}$_i$ and the full-fidelity setting $\boldsymbol{z}^{*}$.
\end{itemize}

This process yields a promising fidelity setting that achieves high correlation with full-fidelity, but comes with lower evaluation cost, enabling reliable yet efficient guidance for the subsequent configuration tuning.

\input{paper_sections/pseudo_fidelity_optimization}

\subsection{Finding Seeds under Imperfect-Fidelity}
\label{subsection:LoFEA}

\tao{I think we need a pair of illustration figures to explain 4.2 and 4.3.}Given a cost-effective fidelity setting $\boldsymbol{z}_{ideal}$ discovered by EvoFD, we next integrate it into evolutionary search to guide the tuning. While $\boldsymbol{z}_{ideal}$ enables cheaper evaluations, directly embedding it into an evolutionary optimizer introduces new challenges. In the context of configuration tuning, a low-fidelity setting, even one selected for its high correlation to full-fidelity, may still mislead the search and fall into local regions due to fidelity loss. This can result in the over-exploitation of suboptimal areas, leading to being trapped in local optima. To address this, LoFEA introduces a two-stage strategy that balances early exploration and stable exploitation. The detailed procedures of LoFEA are illustrated in \textbf{Algorithm~\ref{alg:LoFEA}}.

\subsubsection{Diversity-Preserving Distillation}
To address the above challenges, LoFEA first performs a one-shot sampling and distillation phase. The goal is to collect a set of promising configurations with high diversity and quality, serving as the foundation for subsequent evolution. We proceed as follows:

\begin{itemize}
    \item [(1)] Sample a large number of candidate configurations $\boldsymbol{\mathbfcal{H}}$ from the configuration space $\boldsymbol{\mathbfcal{X}}$ using LHS (line 3).

    
    \item [(2)] Evaluate each configuration $\boldsymbol{x} \in \boldsymbol{\mathbfcal{H}}$ under the low-fidelity setting $\boldsymbol{z}_{ideal}$. 
    Particularly, if $\boldsymbol{x}$ is currently the best-performing configuration under $\boldsymbol{z}_{ideal}$, we trigger a full-fidelity evaluation for $\boldsymbol{x}$ with probability $\alpha$ to progressively collect trustworthy measurements for subsequent tuning (lines 4-11).
    %This selective evaluation helps mitigate false negatives—configurations that may be underestimated by $\boldsymbol{z}_{ideal}$ but perform well under $\boldsymbol{z}^{*}$. 
    %This process continues until the distillation budget $\mathcal{B}_2$ is exhausted (\textbf{lines 4–12}).
    
    \item [(3)] Select the top-$m$ configurations from $\boldsymbol{\mathbfcal{H}}$ (measured under $\boldsymbol{z}_{ideal}$) to form the initial population $\boldsymbol{\mathbfcal{P}}$ for evolution (line 12).
\end{itemize}

Through the above distillation, we can obtain an initial population that balances diversity and quality, which serves as a strong foundation for the subsequent evolutionary search.

\input{paper_sections/pseudo_LoFEA}

\subsubsection{Low-Fidelity Guided Evolution}
With a distilled population $\boldsymbol{\mathbfcal{P}}$ offering diverse and potentially promising configurations, LoFEA performs evolutionary search under the guidance of selected low-fidelity setting $\boldsymbol{z}_{ideal}$ (lines 15-28). In each generation, the configuration offspring $\boldsymbol{\mathbfcal{O}}$ is generated through selection, crossover, and mutation operators. These offspring are measured at fidelity setting $\boldsymbol{z}_{ideal}$, and combined with the current population $\boldsymbol{\mathbfcal{P}}$. Then, the top-$m$ configurations are retained as the parent of the next generation, where $m$ is the population size. This process iterates until the evolution budget $\mathcal{B}_3$ is exhausted.

Notably, to strengthen the robustness of search under low-fidelity guidance, LoFEA incorporates selective full-fidelity evaluation at two critical points. First, the initial $\boldsymbol{\mathbfcal{P}}$ is fully evaluated under $\boldsymbol{z}^{*}$ before evolution begins (line 14). This protects high-potential configurations from being discarded during low-fidelity guided evolution. Second, in each generation, the current best configuration, if not yet evaluated under $\boldsymbol{z}^{*}$, is promoted to full-fidelity evaluation (lines 25-27). These selective probes serve three purposes: (i) they progressively construct a set of trustworthy anchor points across the configuration space to alleviate low-fidelity uncertainty; (ii) they offer a cost-effective strategy to detect high-quality configurations early, without incurring large-scale full-fidelity evaluations; and (iii) they provide HiFEA with a strong warm-start by supplying reliable high-fidelity samples for subsequent tuning.


%The first stage aims to preserve diversity by distilling promising candidates from a wide region of the configuration space, while the second stage performs evolutionary search guided by low-fidelity evaluations with intermittent high-fidelity validation. This design enhances the robustness of the optimizer by reducing the risk of being misled by fidelity noise.



\subsection{Assuring under Perfect-Fidelity with Seeds}
\label{subsection:HiFEA}
\tao{Is this happening iteratively during the low fidelity evolution? Or only at the end of the entire tuning?}
\yulong{This only happens at the end of the entire tuning, but full-fidelity evaluation could be triggered during LoFEA.}
To further consolidate the tuning process under the most reliable evaluation setting, HiFEA performs an evolutionary search entirely guided by the full-fidelity setting $\boldsymbol{z}^{*}$. We begin by promoting all configurations in population $\boldsymbol{\mathbfcal{P}}$ optimized by LoFEA to full-fidelity evaluation and merge them with the trusted set $\boldsymbol{\mathbfcal{V}}$ (measured under $\boldsymbol{z}^{*}$) collected during selective probing. From this combined pool $\boldsymbol{\mathbfcal{P}}$ $\cup$ $\boldsymbol{\mathbfcal{V}}$, the top-$m$ configurations are selected to form the initial configuration population for full-fidelity evolution. Subsequently, HiFEA proceeds with an evolutionary search analogous to LoFEA, iteratively generating offspring through selection, crossover, and mutation operators, but with all evaluations performed under the full-fidelity setting $\boldsymbol{z}^*$. This process continues until the budget $\mathcal{B}_4$ is exhausted, after which the best configuration $\boldsymbol{x}_{best}$ is returned.

This final stage plays a pivotal role in ensuring the credibility and deployability of the output. While earlier phases rely on approximate evaluations for cost efficiency, HiFEA eliminates fidelity loss and corrects ranking deviations by shifting entirely to the full-fidelity evaluation. It enables a rigorous comparison under the most trustworthy setting, ultimately identifying a configuration that is not only high-performing but also reliable enough to be deployed in real systems.










==> paper_sections/metrics.tex <==

\section{Introduction}
\label{section:introduction}


\subsection{Landscape Metrics}
\label{subsection: Landscape Metrics}

\subsubsection{Fitness Distance Correlation (FDC)}
FDC is a widely used metric for evaluating the relationship between the fitness (e.g., runtime and throughput) of solutions (i.e., configurations) and their distance to the global optimum in a given landscape~\cite{jones1995fitness}. It helps to characterize the global structure of the fitness landscape and evaluate the ease or difficulty of navigating toward the global optimum. Formally, FDC is calculated as:

\begin{equation}
\varrho(f, d)=\frac{1}{\sigma_f \sigma_d} \frac{1}{s}\sum_{i=1}^s\left(f_i-\bar{f}\right)\left(d_i-\bar{d}\right),
\end{equation}
where $s$ is the number of solutions considered in FDC. Within such a solutions set, $d_i$ denotes the distance of $i$th solution to the nearest global optimum. $\bar{f}$ ($\bar{d}$) and $\sigma_f$ ($\sigma_d$) are the mean and standard deviation of fitness (and distance). 

%For minimization problems, their can be roughly categorized into three classes based on FDC ($\varrho$) values~\cite{jones1995fitness}:

% \begin{itemize}
%     \item\textbf{\textit{Straightforward}} ($\varrho$ $\geq$ 0.15), in which fitness tends to decrease with distance from the global optimum, guiding the search towards the optimal solution.
%     \item \textbf{\textit{Difficult}} ($\mathcal{-}0.15 \textless \varrho \textless 0.15$), in which there is a trivial correlation between fitness and distance from global optima.
%     \item \textbf{\textit{Misleading}} ($\varrho \leq \mathcal{-} 0.15$), in which fitness tends to increase with distance from the global optimum, misleading the search.
% \end{itemize}

%Following this classification, FDC provides valuable insights into the structural properties of software systems' performance landscapes. By quantifying the relationship between configuration quality and proximity to the optimal solution, FDC helps practitioners in understanding the properties hidden inside the system. 


%Particularly, in this study, the only exception is the \textsc{h2} system, which is a maximization problem focused on maximizing throughput. To ensure consistency in calculating the FDC value, we invert the performance values for the \textsc{h2} system. This adjustment allows for a standardized interpretation of FDC across all studied systems.

%Hence, FDC is an effective measure for evaluating the global landscape structure, evolvability, and potential deception with optimization problems.





\subsubsection{Local optima} Local optima capture the underlying local structural properties of a problem's landscape. Formally, a configuration \textbf{\textit{c}}$^{\ell}$ is considered as a local optima if $f(\textbf{\textit{c}}^{\ell})$ is better than $f(\textbf{\textit{c}})$, $\forall \textbf{\textit{c}} \in \mathcal{N}\left(\textbf{\textit{c}}^{\ell}\right)$, where $\mathcal{N}\left(\textbf{\textit{c}}^{\ell}\right)$ is the neighborhood of \textbf{\textit{c}}$^{\ell}$. Two key aspects are considered when analyzing local optima: (1) the number of local optima; and (2) the quality of local optima.


(1) \textit{The number of local optima} reflects landscape multimodality, indicating the presence of multiple high-performing regions and complexity of the problem. To quantify this, we define $\ell_p$ as the proportion of local optima among all sampled configurations:
\begin{equation}
    \ell_p = \frac{|\mathcal{L}|}{\mathcal{|S|}},
\end{equation}
where $\mathcal{L}$ and $\mathcal{S}$ denote the sets of local optima and all sampled configurations, respectively.

(2) \textit{The quality of local optima}---particularly their relative performance compared to the global optima---indicates the prominence of local peaks and the susceptibility of the landscape to trapping suboptimal solutions. For minimization problems, we define the relative quality of local optima as:
    
\begin{equation}
\ell_q = \frac{\frac{1}{|\mathcal{S}|} \sum\limits_{\textbf{\textit{c}} \in S} f(\textbf{\textit{c}}) - \frac{1}{|\mathcal{L}|} \sum\limits_{\textbf{\textit{c}}^\ell \in \mathcal{L}} f(\textbf{\textit{c}}^\ell)}
{\frac{1}{|\mathcal{S}|} \sum\limits_{\textbf{\textit{c}} \in \mathcal{S}} f(\textbf{\textit{c}}) - f(\textbf{\textit{c}}^g)},
\end{equation}
where $\textbf{\textit{c}}^g$ represents the global optimum, and $\textbf{\textit{c}}^\ell$ denotes a local optima from $\mathcal{L}$. A higher $\ell_q$ indicates that local optima are of higher quality, being closer to the global optimum, while a lower $\ell_q$ suggests an abundance of low-quality local optima.

% \begin{itemize}
%     \item[1)] \textbf{\textit{The number of local optima}} provides insight into the landscape's multimodality, revealing the extent to which multiple distinct regions of relatively superior performance exist. This multimodality reflects the inherent complexity of the problem and the potential for diverse, competing solutions. To provide a more intuitive measure, we introduce $\ell_p$, which represents the proportion of local optima relative to all sampled configurations in a landscape, as follows:
%     \begin{equation}
%         \ell_p = \frac{|\mathcal{L}|}{\mathcal{|S|}},
%     \end{equation}
%     where $\mathcal{L}$ and $\mathcal{S}$ denote the sets of local optima and all sampled configurations, respectively.
    
%     \item[2)] \textbf{\textit{The quality of local optima}}---particularly their relative performance compared to the global optima---indicates the prominence of local peaks and the susceptibility of the landscape to trapping suboptimal solutions. For minimization problems, we define the relative quality of local optima as:
    
%     \begin{equation}
%     \ell_q = \frac{\frac{1}{|\mathcal{S}|} \sum\limits_{\textbf{\textit{c}} \in S} f(\textbf{\textit{c}}) - \frac{1}{|\mathcal{L}|} \sum\limits_{\textbf{\textit{c}}^\ell \in \mathcal{L}} f(\textbf{\textit{c}}^\ell)}
%     {\frac{1}{|\mathcal{S}|} \sum\limits_{\textbf{\textit{c}} \in \mathcal{S}} f(\textbf{\textit{c}}) - f(\textbf{\textit{c}}^g)},
%     \end{equation}
%     where $\textbf{\textit{c}}^g$ represents the global optimum, and $\textbf{\textit{c}}^\ell$ denotes a local optima from $\mathcal{L}$. A higher $\ell_q$ value indicates that local optima exhibit high overall quality, as their performance is closer to the global optimum. In contrast, a lower $\ell_q$ suggests the presence of many low-quality local optima, making optimization more challenging.
% \end{itemize}




\subsubsection{Basin of attraction}
The basin of attraction of a local optimum \( \textbf{\textit{c}}^\ell \), denoted as \( \mathcal{B}(\textbf{\textit{c}}^\ell) \), is the set of all configurations that converge to \( \textbf{\textit{c}}^\ell \) under a local search process. Formally, it can be defined as:

\begin{equation}
\mathcal{B}(\textbf{\textit{c}}^\ell) = \{ \textbf{\textit{c}} \in \mathcal{C} \mid \text{LocalSearch}(\textbf{\textit{c}}) \to \textbf{\textit{c}}^\ell \}.
\end{equation}


%, providing insights into the structural continuity of the landscape surface
\subsubsection{Autocorrelation}
Autocorrelation quantifies the ruggedness of a fitness landscape by measuring how fitness values change across neighboring configurations. Formally, it is defined as:

\begin{equation}
\label{eq:autocorrelation}
r(d) =\frac{\sum_{i=1}^{N-d}\left(f\left(\textbf{\textit{c}}_i\right)-\bar{f}\right)\left(f\left(\textbf{\textit{c}}_{i+d}\right)-\bar{f}\right)}{\sum_{i=1}^{N-d}\left(f\left(\textbf{\textit{c}}_i\right)-\bar{f}\right)^2},
\end{equation}
where $f(\textbf{\textit{c}}_i)$ is the fitness of $i$th visited configuration $\textbf{\textit{c}}_i$ in the random walk~\cite{tavares2008multidimensional}, $\textbf{\textit{c}}_{i+d}$ is the next visited neighbor at step size $d$, and $N$ is the walk length. A high $r(d)$ indicates a smooth landscape, where similar configurations yield comparable fitness values, while a low autocorrelation suggests a rugged landscape with abrupt fitness variations.




==> paper_sections/section_threats_to_validity.tex <==
\section{Threats to Validity}
\label{section:threats_to_validity}

\revision{\textbf{Internal threats} to validity could be raised from the parameter setting of $\alpha$, which controls the probability of triggering full-fidelity evaluations during low-fidelity guided tuning. In our study, we set $\alpha = 0.5$, following empirical evidence from our sensitivity analysis (\textbf{RQ3}), where this value offered a favorable balance between exploration cost and evaluation reliability. Similarly, parameter $l$ controls the number of paired configurations for estimating fidelity perfection. We set $l=10$ to strike a trade-off between estimation reliability and discovery cost: a large $l$ may provide a more reliable estimate but also incurs higher cost for fidelity discovery. Nevertheless, we recognize that the best value of these parameters may vary across systems, and exploring alternative settings could further enhance robustness.}

% \revision{Threats to \textbf{construct validity} primarily concern the chosen evaluation metrics. In this study, we assess commonly used metrics, including efficiency and performance of the best identified configuration. Additionally, we employ the Scott-Knott ESD test to confirm the statistical significance of our results.}

% \revision{\textbf{External threats} to validity mainly arise from the choice of subject systems and the potential impact of runtime noise (e.g., CPU scheduling and I/O contention). To mitigate these concerns, we evaluate \approach~on six systems with diverse characteristics, against 10 state-of-the-art tuners. This broad coverage enhances the generalizability of our findings, though additional systems could further strengthen external validity.} 

% All experiments were conducted in a consistent environment, with each subject system and tuner deployed in isolated Docker containers to minimize interference and control runtime noise. While minor system-level fluctuations are inevitable, fairness was ensured by running all tuners 10 times under identical experimental conditions.

==> tables/notation.tex <==

\begin{tabular}{ll|lll}
\toprule
\textbf{Notation}                                          & \textbf{Description}                                                                                                                                             & \textbf{Notation}                                  & \textbf{Description}                                                                                       &  \\ \midrule
$\mathcal{B}$                                              & Total tuning budget                                                                                                                                              & $\boldsymbol{\mathbfcal{Q}}$                         & The parent of fidelity population in fidelity discovery                                                    &  \\
\cellcolor[HTML]{E5E6FF}$\mathcal{B}_1$                    & \cellcolor[HTML]{E5E6FF}Budget allocated for evolutionary fidelity discovery                                                                                     & \cellcolor[HTML]{E5E6FF}$\boldsymbol{\mathbfcal{W}}$ & \cellcolor[HTML]{E5E6FF}The offspring of fidelity population in fidelity discovery                         &  \\
$\mathcal{B}_2$                                            & Budget allocated for diversity-preserving distillation                                                                                                           & $\rho_{\boldsymbol{z}}$                            & The quantified fidelity level of fidelity setting z                                                        &  \\
\cellcolor[HTML]{E5E6FF}$\mathcal{B}_3$                    & \cellcolor[HTML]{E5E6FF}Budget allocated for low-fidelity guided evolution                                                                                       & \cellcolor[HTML]{E5E6FF}$\tau_{\boldsymbol{z}}$    & \cellcolor[HTML]{E5E6FF}The quantified evaluation cost associated with fidelity   setting $\boldsymbol{z}$ &  \\
$\mathcal{B}_4$                                            & Budget allocated for high-fidelity evolutionary assurer                                                                                                          & $\boldsymbol{z}_{ideal}$                            & The cost-effective low-fidelity setting identified by   evolutionary fidelity discovery                    &  \\
\cellcolor[HTML]{E5E6FF}$\boldsymbol{z}$                   & \cellcolor[HTML]{E5E6FF}A low-fidelity setting (generic)                                                                                                         & \cellcolor[HTML]{E5E6FF}$\alpha$                   & \cellcolor[HTML]{E5E6FF}Probability of triggering high-fidelity evaluation during   low-fidelity tuning    &  \\
$\boldsymbol{z}^*$                                         & The full-fidelity setting                                                                                                                                        & $\boldsymbol{\mathbfcal{H}}$                         & A large candidate pool of candidate configuration samples                                                  &  \\
\cellcolor[HTML]{E5E6FF}$\boldsymbol{\mathbfcal{S}}$         & \cellcolor[HTML]{E5E6FF}A set of $l$ configuration samples used for fidelity   quantification                                                                    & \cellcolor[HTML]{E5E6FF}$m$                        & \cellcolor[HTML]{E5E6FF}The size of configuration population in evolutionary search                        &  \\
$\mathbfcal{F}_{\boldsymbol{z}}$                           & The set of performance evaluations for configurations  in $\boldsymbol{\mathcal{S}}$ under a   low-fidelity setting $\boldsymbol{z}$                             & $\boldsymbol{\mathbfcal{P}}$                         & The parent of configuration population during tuning                                                       &  \\
\cellcolor[HTML]{E5E6FF}$\mathbfcal{F}_{\boldsymbol{z}^*}$ & \cellcolor[HTML]{E5E6FF}The set of performance evaluations for configurations in   $\boldsymbol{\mathcal{S}}$ under the full-fidelity setting $\boldsymbol{z}^*$ & \cellcolor[HTML]{E5E6FF}$\boldsymbol{\mathbfcal{O}}$ & \cellcolor[HTML]{E5E6FF}The offspring of configuration population during tuning                            &  \\
$n$                                                        & The size of fidelity population for fidelity discovery                                                                                                           & $\boldsymbol{\mathbfcal{V}}$                         & The set of configurations evaluated under full-fidelity   setting $\boldsymbol{z}^*$                       &  \\ \bottomrule
\end{tabular}


==> tables/workload_settings.tex <==

\begin{tabular}{l|l|l|l}
\toprule
\textbf{Benchmark}                 & \multicolumn{1}{c|}{Sysbench} & \multicolumn{1}{c|}{Wrk} & \multicolumn{1}{c}{Csmith} \\ \midrule
\textbf{Dimension} & \multicolumn{1}{c|}{5}    & \multicolumn{1}{c|}{4}   & \multicolumn{1}{c}{5}              \\ \midrule
\multirow{5}{*}{\textbf{Factor}} & \texttt{time}: 180            & \texttt{post}: true      & \texttt{max-funcs}: 50     \\
                   & \texttt{tables}: 50        & \texttt{threads}: 8      & \texttt{max-block-size}: 4         \\
                   & \texttt{threads}: 4       & \texttt{duration}: 180   & \texttt{max-block-depth}: 6        \\
                   & \texttt{r/w ratio}: 1:1   & \texttt{connections}: 50 & \texttt{inline-function-prob}: 10  \\
                   & \texttt{table-size}: 100k & \multicolumn{1}{c|}{—}   & \texttt{max-array-len-per-dim}: 50 \\ \bottomrule
\end{tabular}

